In Defense of Scene Graphs for Image Captioning

The mainstream image captioning models rely on Convolutional Neural Network (CNN) image features to generate captions via recurrent models. Recently, image scene graphs have been used to augment captioning models so as to leverage their structural semantics, such as object entities, relationships and attributes. Several studies have noted that the naive use of scene graphs from a black-box scene graph generator harms image captioning performance and that scene graph-based captioning models have to incur the overhead of explicit use of image features to generate decent captions. Addressing these challenges, we propose \textbf{SG2Caps}, a framework that utilizes only the scene graph labels for competitive image captioning performance. The basic idea is to close the semantic gap between the two scene graphs - one derived from the input image and the other from its caption. In order to achieve this, we leverage the spatial location of objects and the Human-Object-Interaction (HOI) labels as an additional HOI graph. SG2Caps outperforms existing scene graph-only captioning models by a large margin, indicating scene graphs as a promising representation for image captioning. Direct utilization of scene graph labels avoids expensive graph convolutions over high-dimensional CNN features resulting in 49% fewer trainable parameters. Our code is available at: https://github.com/Kien085/SG2Caps

==> tex/impact_statement.tex <==
Visual content on the web or from photographs can be made more accessible to visually impaired people via automatic image captioning combined with text-to-speech. 
% Image captioning has also been found useful in providing assistance for generating diagnostics from X-ray images ~\cite{shin2016learning}. 
Industries like commerce, education, digital libraries, and web searching, social media platforms utilize image captioning to mine the visual content for image indexing, image retrieval, and data summarization ~\cite{Kim2014JointSO}. 
Although this helps managing online content and may provide value to the users, it can also compromise the users' privacy. e.g. summarizing user behavior or preferences for targeted advertisement.  
Importantly, image captioning algorithms are still limited by dataset biases and the availability of exhaustive human annotations ~\cite{Burns2018WomenAS}. 
In this paper, we attempt to address the later 
% unavailability of exhaustive annotation and dataset bias ~\cite{Burns2018WomenAS} of captioning dataset 
by leveraging annotations beyond the paired training data via explicit use of scene graphs. More research is necessary to reach human-level accuracy and diversity. 


% Reference impact statements from 2 NeurIPS papers on image captioning:
% [1] https://proceedings.neurips.cc/paper/2020/file/c2964caac096f26db222cb325aa267cb-Paper.pdf
% [2] https://proceedings.neurips.cc/paper/2020/file/24bea84d52e6a1f8025e313c2ffff50a-Paper.pdf

